Block3D: Efficient Text-to-3D Generation via Block-Wise Diffusion

While text-to-3D generation has advanced rapidly, achieving high geometric fidelity at low inference cost remains challenging. Existing text-to-3D methods either decode discrete shape tokens autoregressively or iteratively refine global 3D representations with diffusion or flow models. However, autoregressive decoding is sequential and cannot revise errors, whereas diffusion and flow-matching models repeatedly process the full representation, making high-quality generation increasingly expensive. In this paper, we propose Block3D, a block-wise diffusion framework that partitions the discrete shape-token sequence into contiguous blocks, generates the blocks autoregressively, and jointly denoises all tokens within the current block. To alleviate error accumulation, we introduce confidence-guided intra-block correction, which revises low-confidence tokens before each block is finalized. On a held-out set from TRELLIS-500K, Block3D reduces mean end-to-end generation time from 25.71 seconds to 4.99 seconds, achieving a $5.15\times$ speedup over the fine-tuned autoregressive baseline without sacrificing geometric fidelity.

==> sections/paper_body.tex <==
\section{Introduction}

High-quality 3D assets are increasingly required in game development, film production, virtual and augmented reality, robotics, and embodied AI, creating a growing demand for systems that can generate 3D content from natural-language descriptions. Recent methods have substantially improved the fidelity and diversity of generated assets by learning effective 3D representations~\cite{xiang2025trellis,zhao2025hunyuan3d2,yang2025pandora3d,bhat2025cube,ye2025shapellmomni}. Despite this progress, generating high-fidelity geometry typically requires autoregressive methods to sequentially decode long shape-token sequences or diffusion methods to repeatedly refine the complete latent representation over multiple denoising steps. As the representation becomes more detailed, both choices increase inference cost. Consequently, existing methods still struggle to achieve high geometric quality and low generation latency at the same time.

\begin{wrapfigure}{r}{0.49\textwidth}
    \vspace{-0.6\baselineskip}
    \centering
    \includegraphics[width=\linewidth]{figures/concept.png}
    \captionsetup{width=\linewidth,font=footnotesize}
    \caption{\textbf{Comparison of 3D token generation schedules.}
    (a) Token-wise generation predicts one shape token at a time and cannot revise emitted tokens.
    (b) Full-sequence denoising updates all positions in parallel but repeatedly processes the complete representation.
    (c) Block3D generates blocks from left to right and denoises all positions in the current block in parallel; a filled token can still be corrected before its block is finalized.}
    \label{fig:concept}
    \vspace{-0.6\baselineskip}
\end{wrapfigure}

In this paper, we propose Block3D, a block-wise autoregressive diffusion framework for efficient text-to-3D generation. Its central idea is to shift the causal dependency of autoregressive generation from individual shape tokens to contiguous latent blocks. Blocks are generated causally from left to right, while all tokens within the current block are jointly denoised under bidirectional attention. To preserve geometric fidelity when predicting all tokens within a block in parallel, our confidence-guided correction mechanism not only fills masked positions but also revises low-confidence tokens before the current block is finalized. Consequently, Block3D substantially reduces end-to-end generation latency while alleviating error accumulation within each block. Experiments on 100 held-out objects show that Block3D achieves the best geometric metrics among the evaluated methods while reducing the mean end-to-end generation time from $25.71$ seconds to $4.99$ seconds compared with the separately fine-tuned Cube~\cite{bhat2025cube} baseline, achieving a $5.15\times$ speedup.


Recent work has pursued different efficiency strategies within diffusion/flow and autoregressive generation. Diffusion and flow models avoid token-wise decoding by refining multiple latent variables in parallel. TRELLIS, Hunyuan3D~2.0, and Pandora3D reduce the state being refined through compressed 3D latents, while TSSR denoises the complete mesh-token sequence and PartDiffuser limits each denoising stage to a semantic part~\cite{xiang2025trellis,zhao2025hunyuan3d2,yang2025pandora3d,song2025tssr,yang2026partdiffuser}. These designs reduce the representation size or the active denoising region, but detailed geometry still requires repeated refinement; full-sequence denoising revisits every token, whereas part-wise denoising additionally relies on point-cloud conditioning and semantic part segmentation. Autoregressive generators instead reduce sequential cost by organizing geometry into adaptive, hierarchical, or local units. Adaptive octree tokenization allocates tokens according to geometric complexity, PointNSP and OctGPT generate geometry progressively across spatial scales, TreeMeshGPT follows triangle adjacency, and MeshMosaic generates and assembles local mesh patches~\cite{deng2025octreetokenization,meng2025pointnsp,wei2025octgpt,lionar2025treemeshgpt,xu2025meshmosaic}. Although these representations shorten the causal sequence or its individual dependencies, fine geometry still requires additional tokens, hierarchy levels, branches, or patches to be generated sequentially. Consequently, high-fidelity generation continues to involve repeated latent refinement in diffusion-based methods or substantial sequential decoding in autoregressive methods, making low-latency generation difficult to achieve.

In summary, our main contributions are as follows:
\begin{itemize}
    \item We introduce Block3D, which shifts the causal dependency in Cube~\cite{bhat2025cube} from individual shape tokens to latent blocks and performs parallel denoising within each block, substantially reducing sequential generation latency.
    \item We introduce confidence-guided intra-block correction, which combines mask-to-token recovery with token-to-token editing~\cite{bie2026llada21} to alleviate error accumulation before the current block is finalized.
    \item Experiments on 100 held-out objects show that Block3D achieves the best geometric metrics among the evaluated methods and reduces mean end-to-end generation time from $25.71$ seconds to $4.99$ seconds relative to the fine-tuned Cube~\cite{bhat2025cube} baseline.
\end{itemize}

\section{Related Work}

\subsection{Diffusion-based 3D Generation.}
Diffusion and flow matching support several distinct text-to-3D paradigms. DreamFusion, Magic3D, and MOC-3D optimize a 3D representation with supervision derived from pretrained 2D diffusion models~\cite{poole2022dreamfusion,lin2023magic3d,fan2026moc3d}. Shap-E and Rodin instead diffuse learned 3D representations, while TRELLIS performs flow matching over structured 3D latents~\cite{jun2023shap,wang2023rodin,xiang2025trellis}. Hunyuan3D~2.0, Pandora3D, and CraftsMan3D use staged or native 3D generation pipelines for detailed assets~\cite{zhao2025hunyuan3d2,yang2025pandora3d,wang2024craftsman}. LGM directly predicts 3D Gaussians from multi-view images, whereas DreamCS and VLM3D study learned or vision-language reward signals~\cite{tang2024lgm,zou2025dreamcs,bai2025vlm3d}. These systems should therefore not be grouped under a single VAE-plus-latent-diffusion formulation.

Recent work reduces optimization cost or improves view consistency through iterative reconstruction, flow distillation, direct trajectory design, and multi-view memory~\cite{chen2024microdreamer,yan2025consistent,li2025walking,zhou2025consdreamer,yang2025bridging,zhou2026stream3d}. These approaches update a global, implicit, or multi-view representation. Block3D instead retains a fixed discrete 3D representation and shortens the sequential horizon of its learned prior without changing the tokenizer or mesh decoder.

\subsection{AR-based 3D Generation.}
Another line of work formulates 3D generation as sequence prediction. MeshGPT autoregressively generates quantized triangle sequences, whereas Cube represents a shape by a compact, fixed-length sequence of VQ codes~\cite{siddiqui2024meshgpt,bhat2025cube}. MeshAnything, MeshAnything~V2, MeshRipple, and HiFi-Mesh improve mesh tokenization or shorten local autoregressive dependence~\cite{chen2024meshanything,chen2024meshanythingv2,lin2025meshripple,li2026hifimesh}. LLaMA-Mesh serializes vertices and faces as text tokens for a language model~\cite{wang2024llamamesh}. ShapeLLM targets language-grounded 3D understanding, while ShapeLLM-Omni extends multimodal language modeling to both understanding and generation~\cite{qi2024shapellm,ye2025shapellmomni}. VAR-3D introduces a view-aware 3D tokenizer, and AR3D-R1 studies reinforcement learning for autoregressive text-to-3D generation~\cite{han2025var3d,tang2025ar3dr1}.

Token-wise autoregression incurs one sequential decision per code and makes every emitted code irreversible. Later predictions are consequently conditioned on generated rather than ground-truth prefixes, the standard exposure-bias setting~\cite{bengio2015scheduled,ranzato2015sequence}. Block3D does not remove generated-prefix exposure bias: completed blocks remain fixed. It provides only a bounded opportunity to revise codes within the active block before that block becomes part of the prefix.

\subsection{Block-wise and Editable Decoding.}
Discrete denoising models replace continuous Gaussian noise with categorical transitions, while masked generators iteratively reveal token subsets with bidirectional context~\cite{austin2021structured,chang2022maskgit}. In 3D generation, PartDiffuser uses semantic mesh parts as causal groups and denoises tokens within each part, whereas TSSR performs global discrete mesh-token generation followed by remasking-based refinement~\cite{yang2026partdiffuser,song2025tssr}. Block3D differs from both by operating on part-free, fixed-length Cube~\cite{bhat2025cube} codes and freezing every completed prefix block.

Block Diffusion establishes autoregressive factorization across blocks, bidirectional denoising within the active block, clean/noisy training attention, and prefix caching~\cite{arriola2025blockdiffusion}. Subsequent systems study efficient block-diffusion language decoding, vision-language tokens, sparse attention, and vision-language-action generation~\cite{wu2025fastdllmv2,cheng2025sdarvl,xi2026losa,wang2026blockvla,lee2026tbdvla}. LLaDA2.1 introduces M2T/T2T editing and mixed mask/random-token supervision with multi-turn-forward augmentation~\cite{bie2026llada21}. Block3D adopts these established mechanisms but specifies the sample-level mixture, shape-code corruption, residual objective, confidence-gated updates, and deterministic quota for fixed-length 3D codes. The resulting T2T operation is restricted to the active block and executed within the fixed decoding horizon; Appendix Section~A.4 gives the complete update procedure.

\section{Method}
\label{sec:method}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{sections/pipeline_02.png}
    \caption{\textbf{Block3D overview.} Text and optional bounding-box conditions guide left-to-right block generation. Completed blocks form a frozen causal prefix, while M2T and T2T~\cite{bie2026llada21} edit only the active block before the frozen decoder maps the completed codes to a mesh.}
    \label{fig:pipeline}
\end{figure}

\subsection{Overview}
\label{sec:method_overview}

Figure~\ref{fig:pipeline} shows the complete text-to-mesh pipeline. We use the frozen VQ autoencoder of Cube~\cite{bhat2025cube}, which represents each mesh with $N=1024$ discrete codes from a codebook of size $V=16384$ and decodes a completed code sequence back to a mesh. Given a prompt $y$, a frozen CLIP ViT-L/14 text encoder~\cite{radford2021learning} produces 77 token-level features; an optional projected bounding-box token can be appended, although every reported experiment uses text alone. The resulting condition $C$ drives the Cube-initialized generator. The $N$ shape-code positions are divided into $K$ contiguous blocks. Generation follows the block-causal schedule of Block Diffusion~\cite{arriola2025blockdiffusion}: the current block starts fully masked, attends to the condition and the committed prefix, and predicts all active positions in parallel. Within that block, the M2T and T2T updates adapted from LLaDA2.1~\cite{bie2026llada21} fill masked positions and revise already filled positions before commitment. The completed block is then frozen and added to the cached prefix, and the same process continues from left to right. After all $K$ blocks are committed, the frozen VQ decoder converts the completed code sequence $\hat{x}$ into the output mesh $\hat{S}$.

The method has three components. \textbf{(1) Conditioned block-causal denoising} partitions the fixed-length shape sequence into contiguous computational blocks, defines the clean/corrupted training visibility, and restricts bidirectional attention to the active block. \textbf{(2) Edit-aware training} exposes the generator to both masked and substituted shape codes, applies one model-based rollout, and supervises only the residual errors after that rollout. \textbf{(3) Bounded confidence-guided decoding} uses conditional confidence for M2T filling and T2T replacement~\cite{bie2026llada21}, while a deterministic reveal quota guarantees that every mask is removed within at most $T$ iterations, where $T$ is the per-block update horizon. The first component transfers block-causal generation to fixed-length 3D codes; the latter two specify how editable states are trained and completed under a fixed inference horizon. All revisions remain intra-block because committed prefix blocks are never reopened.

\subsection{Block-Causal Shape-Code Denoising}
\label{sec:block_generation}

The conditional prior retains the DualStream RoFormer generator of Cube~\cite{bhat2025cube}. We write its shape-code logits as $\ell=F_\theta(C,z;A,p)$, where $z$ is the visible shape state, $A$ is its attention mask, and $p$ gives the logical position indices. Probabilities and generated codes use only the first $V$ output entries. The auxiliary mask $[M]$ reuses the inherited padding-token identifier for input embedding lookup, but it is excluded from output normalization and is never passed to the frozen shape decoder.

Let the block size $B$ and denoising horizon $T$ be positive integers. We form $K=\lceil N/B\rceil$ contiguous blocks. Block $k$ contains the positions $I_k=\{(k-1)B+1,\ldots,\min(kB,N)\}$ for $k=1,\ldots,K$, so only the final block can contain fewer than $B$ codes.
Writing $x^{(k)}=x_{I_k}$, $\hat{x}^{(k)}=\hat{x}_{I_k}$, and $\hat{x}^{(<k)}=(\hat{x}^{(1)},\ldots,\hat{x}^{(k-1)})$, the block-causal dependency inherited from Block Diffusion~\cite{arriola2025blockdiffusion} is realized as
\begin{equation}
\hat{x}^{(k)}=
\mathcal{G}_{\theta,T}\!\left(\hat{x}^{(<k)},C\right),
\qquad k=1,\ldots,K,
\label{eq:block_transition}
\end{equation}
where $\mathcal{G}_{\theta,T}$ is the deterministic transition in Algorithm~\ref{alg:block3d_sampling}; the other fixed decoding hyperparameters are suppressed from its notation. Equation~(\ref{eq:denoising_loss}) trains the token denoiser used inside this transition; we do not interpret $\mathcal{G}_{\theta,T}$ as an exact block likelihood.

At inference for block $k$, the generator receives $[\hat{x}^{(<k)};z_k]$ on the shape side. Prefix queries use token-causal visibility. Every active-block query attends to the complete prefix and bidirectionally to all positions in $z_k$; future blocks are absent.

Adapting the vectorized clean-and-corrupted construction of Block Diffusion~\cite{arriola2025blockdiffusion} to Cube~\cite{bhat2025cube}, training evaluates all block contexts in one forward pass over the concatenated sequence $[x;\tilde{x}]$. A query in the clean copy can attend only to clean tokens in its own block and all preceding blocks; it cannot attend to a later clean block or any token in the corrupted copy. A query in the corrupted copy can attend to the clean tokens of all preceding blocks and bidirectionally to the corrupted tokens within its own block. It cannot access the clean target tokens of the current block, clean tokens from future blocks, or corrupted tokens from any other block. Every shape query additionally attends to all condition tokens, whereas condition queries attend only to condition tokens. This visibility rule allows the corrupted states of all blocks to be trained in parallel without exposing the clean target of the block being reconstructed.

The two copies share logical positions, $p(x_i)=p(\tilde{x}_i)=i$. At inference, prefix queries use token-causal visibility and active-block queries remain bidirectional. Training thus uses block-bidirectional teacher-forced prefixes, whereas inference uses token-causal generated prefixes. Caching reduces repeated computation~\cite{arriola2025blockdiffusion}, but does not remove this mismatch or exposure bias. Appendix Section~A.2 gives the complete masks and position-ID construction.

\subsection{Edit-Aware Corruption and Training}
\label{sec:training}

LLaDA2.1~\cite{bie2026llada21} motivates supervision on both masked and substituted states but does not determine the shape-code corruption used here. For each training sample and block, we draw $\tau_k\sim\mathcal{U}(t_{\min},t_{\max})$ and independently sample $e_i\sim\mathrm{Bernoulli}(\tau_k)$ for $i\in I_k$. A single sample-level variable $a\sim\mathrm{Bernoulli}(\rho)$ selects the initial corruption stream: $a=0$ is M2T and $a=1$ is T2T. We set
\begin{equation}
\tilde{x}^{(0)}_i=
\left\{
\begin{array}{ll}
[M], & e_i=1,\ a=0,\\
u_i, & e_i=1,\ a=1,\\
x_i, & e_i=0,
\end{array}
\right.
\label{eq:training_corruption}
\end{equation}
where $u_i$ is uniform over the $V-1$ shape codes different from $x_i$. We use $(t_{\min},t_{\max})=(0.45,0.95)$ and $\rho=0.5$. The variables $\tau_k$ control corruption only and are not supplied to $F_\theta$ as time embeddings. Uniform wrong codes diversify substituted-state supervision, while the model-based rollout below introduces model-generated candidates before the residual loss. Inference starts each active block from the all-mask state.

Classifier-free condition dropout~\cite{ho2022classifierfree} is sampled once per batch element before either model evaluation. Let $\bar{C}_n=C_n$ for a retained condition and $\bar{C}_n=C_n^-$ for a dropped condition, where $C_n^-$ contains the empty-text encoding and, when enabled, a zero bounding box. The same realized condition $\bar{C}_n$ is reused by both evaluations below.

Inspired by the multi-turn-forward augmentation of LLaDA2.1~\cite{bie2026llada21}, we instantiate one model-based rollout ($R=1$) before computing the loss. For every block, the rollout initializes $z_k^{(0)}=\tilde{x}^{(0)}_{I_k}$. A no-gradient forward pass on $[x;\tilde{x}^{(0)}]$ supplies unguided logits ($g=0$) under $\bar{C}_n$, after which the update sets in Equations~(\ref{eq:m2t_set})--(\ref{eq:t2t_set}) are applied independently within every corrupted block using $(\eta_M,\eta_T)$ and the first-step quota $q_0$. Under the default $B=64$ and $T=4$, $q_0=16$. The simultaneous updates define $z_k^{(1)}$, and the rollout output is assembled by setting $\tilde{x}^{(R)}_{I_k}=z_k^{(1)}$ for every block. This state may contain masks, correct codes, and model-produced incorrect codes even when its initial state used only one corruption stream.

We then perform a separate gradient-carrying forward pass on $[x;\tilde{x}^{(R)}]$ and retain only corrupted-copy logits. For batch index $n$, let $\pi^{(R)}_{\theta,n,i}$ be their softmax over the first $V$ entries. Under the training visibility rule above, this distribution is conditioned on $\bar{C}_n$, the clean blocks preceding the block that contains position $i$, and the current corrupted block. Over all valid shape positions in the batch, define $\mathcal{D}=\{(n,i):\tilde{x}^{(R)}_{n,i}\neq x_{n,i}\}$. The objective is
\begin{equation}
\mathcal{L}=-\frac{1}{|\mathcal{D}|+\epsilon}
\sum_{(n,i)\in\mathcal{D}}
\log\pi^{(R)}_{\theta,n,i}(x_{n,i}).
\label{eq:denoising_loss}
\end{equation}
We set $\epsilon=10^{-8}$ and reduce over all residual tokens in the batch. Samples without residuals add no term; an empty $\mathcal{D}$ yields zero loss. The one-step rollout adds a generation-dependent state, while preceding blocks remain teacher-forced and cross-block exposure bias remains. Appendix Section~A.3 specifies corruption, rollout ordering, residual reduction, and empty-set handling.

\subsection{Bounded Confidence-Guided Decoding}
\label{sec:inference}

\begin{algorithm}[t]
\caption{Bounded editable block decoding}
\label{alg:block3d_sampling}
\small
\begin{algorithmic}[1]
\REQUIRE Conditional branch $C^+$; unconditional $C^-$ if $g>0$; $B,T,g,\eta_M,\eta_T$
\STATE Initialize $\hat{x}\leftarrow[M]^N$
\FOR{$k=1$ to $K$}
  \STATE Set $z_{k,i}^{(0)}\leftarrow[M]$ for every $i\in I_k$; set $S_k\leftarrow T$
  \STATE Build the batched condition/prefix cache
  \FOR{$s=0$ to $T-1$}
    \STATE Compute $\ell_s^+$ and, if $g>0$, $\ell_s^-$ from active state $z_k^{(s)}$
    \STATE Compute $\hat{z}_s,\alpha_s$ by Equations~(\ref{eq:guided_logits})--(\ref{eq:conditional_confidence})
    \STATE Compute $q_s$ and $\mathcal{M}_s$ from the current active state
    \STATE Form $\mathcal{U}^{\mathrm{M2T}}_s,\mathcal{U}^{\mathrm{T2T}}_s$ by Equations~(\ref{eq:m2t_set})--(\ref{eq:t2t_set})
    \IF{$\mathcal{M}_s=\emptyset$ and both update sets are empty}
      \STATE Set $S_k\leftarrow s$; \textbf{break}
    \ENDIF
    \STATE Compute $z_{k,i}^{(s+1)}$ by Equation~(\ref{eq:state_update}) for every $i\in I_k$
  \ENDFOR
  \STATE Commit $\hat{x}_{I_k}\leftarrow z_k^{(S_k)}$ and freeze block $k$
\ENDFOR
\RETURN the frozen shape decoder output $D_{\mathrm{shape}}(\hat{x})$
\end{algorithmic}
\end{algorithm}


\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{Block3D_demos.jpeg}
    \caption{\textbf{Qualitative Comparison of Text-to-3D Generation.} Compared to existing paradigms, Block3D produces coherent front and back views in these examples, while several baselines exhibit missing or distorted geometry. Complete prompts and the selection protocol are documented in Appendix Section~D.2.}
    \label{fig:qualitative_comp}
\end{figure*}

Let the guidance coefficient satisfy $g\geq0$, and let $\eta_M,\eta_T\in[0,1]$ be the M2T and T2T confidence thresholds~\cite{bie2026llada21}. For block $k$, let $n_k=|I_k|$ and initialize $z_{k,i}^{(0)}=[M]$ for every $i\in I_k$. We suppress $k$ in iteration-level logits and update sets. At iteration $s\in\{0,\ldots,T-1\}$, the conditional branch $C^+$ encodes the prompt, while $C^-$ encodes the empty prompt and, when enabled, a zero bounding box. The branches produce $\ell_s^+$ and $\ell_s^-$. Classifier-free guidance (CFG)~\cite{ho2022classifierfree} gives
\begin{equation}
\ell_s^{g}=(1+\gamma_s)\ell_s^{+}-\gamma_s\ell_s^{-},
\qquad \gamma_s=g\frac{T-s}{T}.
\label{eq:guided_logits}
\end{equation}
Thus the guidance coefficient decreases from $g$ to $g/T$, rather than to zero; when $g=0$, the unconditional branch is omitted and $\ell_s^g=\ell_s^+$. For the deterministic sampler used in our experiments, the candidate and its acceptance confidence are
\begin{equation}
\begin{array}{rcl}
\hat{z}_{s,i}
&=&\mathop{\arg\max}_{0\leq v<V}\ell^g_{s,i,v},\\
\alpha_{s,i}
&=&\mathop{\mathrm{softmax}}(\ell^+_{s,i,0:V-1})[\hat{z}_{s,i}].
\end{array}
\label{eq:conditional_confidence}
\end{equation}
The guided logits propose a shape code, whereas the conditional logits determine whether it is accepted; CFG therefore does not directly inflate the threshold score. Ties in the argmax are resolved by selecting the smallest shape-code index.

We assign each iteration a deterministic minimum reveal quota
\begin{equation}
q_s=\left\lfloor\frac{n_k}{T}\right\rfloor
+\mathbf{1}\!\left[s<n_k\bmod T\right],
\qquad \sum_{s=0}^{T-1}q_s=n_k.
\label{eq:transfer_budget}
\end{equation}
Let $\mathcal{M}_s=\{i\in I_k:z_{k,i}^{(s)}=[M]\}$. Following the editable update in LLaDA2.1~\cite{bie2026llada21}, M2T and T2T select
\begin{equation}
\begin{array}{rcl}
\mathcal{U}^{\mathrm{M2T}}_s
&=&\{i\in\mathcal{M}_s:\alpha_{s,i}>\eta_M\}\\
&&{}\cup\ \mathop{\mathrm{TopK}}\limits_{i\in\mathcal{M}_s}
(\alpha_{s,i},\min(q_s,|\mathcal{M}_s|)),
\end{array}
\label{eq:m2t_set}
\end{equation}
\begin{equation}
\mathcal{U}^{\mathrm{T2T}}_s=
\{i\in I_k\setminus\mathcal{M}_s:\hat{z}_{s,i}\neq z_{k,i}^{(s)},\
\alpha_{s,i}>\eta_T\}.
\label{eq:t2t_set}
\end{equation}
Here, $\mathrm{TopK}_{i\in\mathcal{M}_s}(\alpha_{s,i},r)$ returns the $r$ masked positions with the largest confidence values and returns the empty set when $r=0$. Confidence ties are resolved in ascending order of the global position index $i$. This defines short final blocks and settings with $n_k<T$. Appendix Section~A.4 gives the complete sampler, including tie handling and short-block execution.
The active state is updated simultaneously:
\begin{equation}
z_{k,i}^{(s+1)}=
\left\{
\begin{array}{ll}
\hat{z}_{s,i}, & i\in\mathcal{U}^{\mathrm{M2T}}_s\cup
\mathcal{U}^{\mathrm{T2T}}_s,\\
z_{k,i}^{(s)}, & \mbox{otherwise.}
\end{array}
\right.
\label{eq:state_update}
\end{equation}
High-confidence M2T updates can make the number of revealed positions exceed $q_s$, so $q_s$ is a lower bound on progress rather than an upper update budget. T2T does not inspect the confidence of the old code: it replaces a filled code only when a different new candidate exceeds $\eta_T$.

If $m_s=|\mathcal{M}_s|$, the TopK fallback reveals at least $\min(q_s,m_s)$ masked positions, so Equation~(\ref{eq:m2t_set}) implies $m_{s+1}\leq\max(m_s-q_s,0)$. Applying this bound across iterations and using $\sum_{s=0}^{T-1}q_s=n_k$ gives $m_T=0$. The quota therefore completes every active block within $T$ iterations while confidence-gated T2T editing~\cite{bie2026llada21} remains available at every iteration before commitment.

We retain the 23-layer DualStream RoFormer from Cube~\cite{bhat2025cube} (12 heads, width 1536), bypass its inherited single-stream layer on this path, and initialize the first $V$ token embeddings from a projection of the frozen VQ codebook. We fine-tune only this generator. Inference uses $B=64$, $T=4$, $(\eta_M,\eta_T)=(0.95,0.9)$ for M2T/T2T editing~\cite{bie2026llada21}, and guidance coefficient $g=3.0$ under Equation~(\ref{eq:guided_logits}), giving $K=16$.

With CFG~\cite{ho2022classifierfree}, conditional and unconditional branches are concatenated in the batch. Decoding makes $K$ cache calls and at most $KT$ active-block calls, equivalent to at most $2K(T+1)$ logical branch evaluations when $g>0$; the default uses at most 80 batched or 160 logical calls. Following Block Diffusion~\cite{arriola2025blockdiffusion}, the condition and prefix cache are reused within the $T$ updates and rebuilt after commitment. Thus intra-block revision has a fixed horizon, while completed blocks cannot be corrected. Appendix Section~A.5 gives the cache construction and model-call complexity derivation.

\section{Experiments}

\subsection{Experimental Settings}

\paragraph{Datasets.}
We fine-tune the text-to-shape generator on 300K objects sampled from TRELLIS-500K~\cite{xiang2025trellis}, a large-scale collection of 3D assets with paired text descriptions. To construct the evaluation set, we first randomly select 100 objects from TRELLIS-500K using seed 42 and exclude these exact objects from the fine-tuning candidate pool. Each shape is converted into discrete shape tokens using the frozen Cube~\cite{bhat2025cube} tokenizer, and its paired text serves as the generation condition. Each evaluation object retains its paired text prompt, and every method generates one shape per prompt. Appendix Section~B.1 records the split, identifiers, prompts, and exclusion rule; Appendix Section~B.2 specifies preprocessing.

\paragraph{Baselines and Evaluation Metrics.}

\begin{table}[t]
\centering
\begingroup
\small
\renewcommand{\arraystretch}{1.10}
\begin{tabular}{@{}lcccc@{}}
\toprule
Method & CD-L1$\downarrow$ & NC$\uparrow$ & F@1\%$\uparrow$ & CLIP$\uparrow$ \\
\midrule
ShapeLLM-Omni & 0.229 & 0.490 & 0.089 & 19.08 \\
TRELLIS-text  & 0.222 & 0.496 & 0.090 & 20.41 \\
AR3D-R1       & 0.145 & 0.583 & 0.162 & 21.92 \\
Cube          & 0.094 & 0.632 & 0.219 & \textbf{23.87} \\
Block3D       & \textbf{0.078} & \textbf{0.668} & \textbf{0.309} & 23.24 \\
\bottomrule
\end{tabular}
\endgroup
\caption{Geometry and text-shape alignment on the 100-object TRELLIS-500K~\cite{xiang2025trellis} evaluation set. F@1 denotes an F-score threshold of 1\%~\cite{fan2017pointset,mescheder2019occupancy}. Geometry metrics are rounded to three decimals and CLIPScore~\cite{hessel2021clipscore} to two decimals.}
\label{tab:main_results}
\end{table}

\begin{table}[t]
\centering
\begingroup
\small
\renewcommand{\arraystretch}{1.10}
\begin{tabular}{@{}lcccc@{}}
\toprule
Method & Mean$\downarrow$ & Median$\downarrow$ & P90$\downarrow$ & Std.$\downarrow$ \\
\midrule
TRELLIS-text  & 11.65 & 9.75  & 20.06 & 5.59 \\
ShapeLLM-Omni & 36.89 & 33.69 & 40.64 & 8.48 \\
AR3D-R1       & 79.80 & 82.48 & 94.19 & 17.34 \\
Cube          & 25.71 & 25.43 & 26.68 & 0.80 \\
Block3D       & \textbf{4.99} & \textbf{4.96} & \textbf{5.60} & \textbf{0.43} \\
\bottomrule
\end{tabular}
\endgroup
\caption{End-to-end generation time in seconds over the 100 TRELLIS-500K~\cite{xiang2025trellis} prompts, measured on one NVIDIA A100 80GB GPU.}
\label{tab:efficiency}
\end{table}


We compare Block3D with ShapeLLM-Omni~\cite{ye2025shapellmomni}, TRELLIS-text~\cite{xiang2025trellis}, AR3D-R1~\cite{tang2025ar3dr1}, and Cube~\cite{bhat2025cube}. Cube provides the controlled comparison because both models use the same released checkpoint, frozen geometry components, training subset, and optimization budget; the remaining methods use their official inference settings. Appendix Section~C.4 lists releases and complete baseline settings.

Geometry evaluation samples 8,192 surface points and normals per mesh pair and reports Chamfer-$L_1$ distance, normal consistency, and F-score at 1\% of the target bounding-box diagonal~\cite{fan2017pointset,mescheder2019occupancy}. Eight-view CLIPScore measures text-shape alignment with CLIP ViT-L/14~\cite{hessel2021clipscore,radford2021learning}. Latency statistics are measured on one NVIDIA A100 and include condition encoding, shape-code generation, and mesh decoding, but exclude model loading and disk I/O. Protocol details appear in Appendix Section~C.1 (geometry), C.2 (CLIPScore), C.3 (latency), and C.5 (invalid outputs and statistical scope).

\paragraph{Implementation Details.}
We initialize Block3D from the released Cube~\cite{bhat2025cube} checkpoint and freeze its shape tokenizer, CLIP ViT-L/14~\cite{radford2021learning} text encoder, and shape decoder. Only the text-to-shape generator is fine-tuned. We train for 35K steps with AdamW~\cite{loshchilov2019decoupled}, a learning rate of $1\times10^{-4}$, bfloat16 precision, and a global batch size of 40 on four NVIDIA A100 80GB GPUs. We use a 100-step linear warm-up, zero weight decay, a gradient clipping norm of 1.0, and random seed 42. Appendix Section~B.3 gives the complete training and checkpoint configuration.

During training, the block corruption level is sampled uniformly from $[0.45,0.95]$, the T2T branch~\cite{bie2026llada21} is selected with probability $0.5$, and one no-gradient model-based filling rollout is performed. Classifier-free condition dropout~\cite{ho2022classifierfree} is applied with probability $0.1$. Unless otherwise stated, inference uses a block size of 64, four denoising steps per block, M2T and T2T confidence thresholds of 0.95 and 0.9, and guidance coefficient $g=3.0$ in Equation~(\ref{eq:guided_logits}). With $T=4$, $\gamma_s$ decreases linearly from 3.0 to 0.75 across the four iterations. We use deterministic argmax decoding without top-$p$ sampling. Parameter selection is in Appendix Section~B.4; code and materials are indexed in Appendix Sections~E.1--E.3.

\subsection{Comparison with 3D Generation Methods}

\paragraph{Geometry Metrics Comparison.}
Table~\ref{tab:main_results} compares paired geometric fidelity and text-shape alignment. Under the shared evaluation protocol, Block3D attains the strongest CD-L1, NC, and F@1\% scores~\cite{fan2017pointset,mescheder2019occupancy} among the evaluated methods, while its CLIPScore~\cite{hessel2021clipscore} remains competitive. The controlled comparison with Cube~\cite{bhat2025cube} shows that block-wise denoising improves paired geometric fidelity in addition to accelerating generation.

\begin{table}[t]
\centering
\begingroup
\small
\renewcommand{\arraystretch}{1.10}
\begin{tabular}{@{}lcccc@{}}
\toprule
Model & Time$\downarrow$ & CD-L1$\downarrow$ & NC$\uparrow$ & F@1\%$\uparrow$ \\
\midrule
Block3D ($B=32$)  & 12.98 & \textbf{0.076} & 0.667 & 0.296 \\
Block3D ($B=64$)  & 4.99  & 0.078 & \textbf{0.668} & \textbf{0.309} \\
Block3D ($B=96$)  & 3.62  & 0.085 & 0.660 & 0.279 \\
Block3D ($B=128$) & 2.90  & 0.090 & 0.647 & 0.258 \\
Block3D ($B=256$) & \textbf{2.15} & 0.186 & 0.578 & 0.103 \\
\bottomrule
\end{tabular}
\endgroup
\caption{Effect of block size on Block3D with four denoising steps per block. Time is reported in seconds. Every configuration is trained independently.}
\label{tab:block_ablation}
\end{table}

\begin{table}[t]
\centering
\begingroup
\small
\renewcommand{\arraystretch}{1.10}
\begin{tabular}{@{}lcccc@{}}
\toprule
Model & Time$\downarrow$ & CD-L1$\downarrow$ & NC$\uparrow$ & F@1\%$\uparrow$ \\
\midrule
Block3D ($T=4$)  & \textbf{4.99} & \textbf{0.078} & 0.668 & \textbf{0.309} \\
Block3D ($T=8$)  & 7.33  & 0.079 & 0.665 & 0.300 \\
Block3D ($T=12$) & 9.37  & 0.084 & 0.668 & 0.284 \\
Block3D ($T=20$) & 13.66 & \textbf{0.078} & \textbf{0.676} & 0.303 \\
\bottomrule
\end{tabular}
\endgroup
\caption{Effect of denoising steps on Block3D with a block size of 64. Time is reported in seconds. Every configuration is trained independently.}
\label{tab:step_ablation}
\centering
\begingroup
\small
\renewcommand{\arraystretch}{1.10}
\begin{tabular}{@{}lcccc@{}}
\toprule
Model & CD-L1$\downarrow$ & NC$\uparrow$ & F@1\%$\uparrow$ & CLIP$\uparrow$ \\
\midrule
Block3D (M2T)       & 0.081 & 0.666 & 0.287 & 22.74 \\
Block3D (M2T+T2T)   & \textbf{0.078} & \textbf{0.668} & \textbf{0.309} & \textbf{23.24} \\
\bottomrule
\end{tabular}
\endgroup
\caption{Effect of token-to-token editing~\cite{bie2026llada21}. Geometry metrics are rounded to three decimals and CLIPScore~\cite{hessel2021clipscore} to two decimals.}
\label{tab:t2t_ablation}
\end{table}

\paragraph{Efficiency Metrics Comparison.}
Table~\ref{tab:efficiency} shows that Block3D is the fastest evaluated method across all reported latency statistics. Its mean end-to-end generation time is 4.99 seconds, corresponding to a $5.15\times$ speedup over the controlled Cube~\cite{bhat2025cube} baseline. The consistent improvements in median and P90 latency show that this advantage holds across the 100 TRELLIS-500K~\cite{xiang2025trellis} prompts rather than arising from a small number of easy cases.

\subsection{Ablation Study}

We study block size, the number of denoising steps, and token-to-token editing~\cite{bie2026llada21}. Every configuration in Tables~\ref{tab:block_ablation} and~\ref{tab:step_ablation}, as well as both variants in Table~\ref{tab:t2t_ablation}, is trained independently for the same number of optimization steps and evaluated on the same 100-object TRELLIS-500K~\cite{xiang2025trellis} evaluation set.

\paragraph{Effect of Block Size.}
Table~\ref{tab:block_ablation} shows that larger blocks reduce the number of left-to-right stages but make parallel denoising harder. Moving from $B=64$ to 96 lowers latency from 4.99 to 3.62 seconds but reduces F@1\% from 0.309 to 0.279; at $B=256$, F@1\% falls to 0.103. We therefore use $B=64$ as the quality--latency balance.

\paragraph{Effect of Denoising Steps.}
Table~\ref{tab:step_ablation} shows that additional steps increase latency without monotonic quality gains. At $T=20$, latency rises to 13.66 seconds while CD-L1 remains 0.078 and F@1\% is 0.303, compared with 4.99 seconds and 0.309 at $T=4$. We therefore use four steps.

\paragraph{Effect of Token-to-Token Editing.}
Table~\ref{tab:t2t_ablation} compares the complete model with an independently trained M2T-only variant~\cite{bie2026llada21}. Adding T2T editing reduces CD-L1 by 4.7\%, raises F@1\% from 0.287 to 0.309, and raises CLIPScore from 22.74 to 23.24. The simultaneous gains support token correction for revising errors that mask-only recovery cannot address.

\subsection{Discussion and Limitations}

Block3D combines the frozen Cube representation~\cite{bhat2025cube}, the Block Diffusion schedule~\cite{arriola2025blockdiffusion}, and LLaDA2.1 editing~\cite{bie2026llada21} with shape-code corruption, residual rollout supervision, and confidence-guided active-block revision. Because blocks follow Cube's one-dimensional code order and committed prefixes remain immutable, the method targets intra-block errors rather than semantic-part structure or cross-block exposure bias. Its fixed horizon bounds decoding cost and completes every active block within $T$ steps (Appendix Section~A.4).

\section{Conclusion}

Block3D replaces the token-wise prior of Cube~\cite{bhat2025cube} with block-causal denoising, generating blocks from left to right while jointly denoising and correcting the active shape codes. Among the evaluated methods, it improves paired geometry and reduces Cube's mean generation time from 25.71 to 4.99 seconds while retaining competitive text-shape alignment. Completed blocks remain fixed; future work will study cross-block refinement and broader shape representations and datasets.

